Stubborn: A Strong Baseline for Indoor Object Navigation

We present a strong baseline that surpasses the performance of previously published methods on the Habitat Challenge task of navigating to a target object in indoor environments. Our method is motivated from primary failure modes of prior state-of-the-art: poor exploration, inaccurate object identification, and agent getting trapped due to imprecise map construction. We make three contributions to mitigate these issues: (i) First, we show that existing map-based methods fail to effectively use semantic clues for exploration. We present a semantic-agnostic exploration strategy (called Stubborn) without any learning that surprisingly outperforms prior work. (ii) We propose a strategy for integrating temporal information to improve object identification. (iii) Lastly, due to inaccurate depth observation the agent often gets trapped in small regions. We develop a multi-scale collision map for obstacle identification that mitigates this issue.

==> [IROS 2022] Stubborn_Object_Navigation/backup_related_work.tex <==

\section{Related Work}
\label{sec:related-work}

%Two lines of work have been developed to exploit semantics for efficient exploration: (i) constructing an occupancy map using SLAM~\cite{cadena2016past} where every location is labelled with one out of N predefined semantic categories. Such a map is leveraged to set exploration goals for the agent~\cite{chaplot2020gose,Yang2019scenepriors}. (ii) The second approach is end-to-end and predicts actions directly from the raw RGBD observation, the image segmented into several object categories and other metadata~\cite{ye2021auxiliary,Khandelwal2021objectnav-clip, maksymets2021thda,Mousavian2019VisualRF,Wahid2020objectnav-sac}. 

%To find the goal object in an unseen environment, the agent needs to explore the environment, infer goal object locations, and identify the goal object. We briefly discuss prior work on the task of object navigation, as well as related work on semantic maps and object detection.

\textbf{Object Navigation}
Some recent works have approached object navigation via end-to-end imitation or reinforcement learning approaches while implicitly learning semantic priors within the models. Ye et al.~\cite{ye2021auxiliary} learn a policy via reinforcement learning with auxiliary learning tasks and an exploration reward. Khandelwal et al. \cite{Khandelwal2021objectnav-clip} incorporate Contrastive language image pretraining(CLIP, a type of neural network encoder) features for object navigation. Furthermore, Maksymets et al. \cite{maksymets2021thda} augment scenes by inserting objects to increase object and trajectory diversity during training. Mousavian et al. \cite{Mousavian2019VisualRF} use imitation learning to learn a policy. Wahid et al. \cite{Wahid2020objectnav-sac} address the similar problem of object navigation with continuous control using Soft Actor-Critic \cite{Haarnoja2018SAC}.

In contrast, other works have built explicit spatial representations that are then used in navigation, such as a map of the explored region in Simultaneous Localization And Mapping\cite{durrant2006simultaneous}. Chaplot et al. \cite{chaplot2020gose} propose a hierarchical SLAM-based approach, winning the 2020 iteration of the Habitat Challenge \cite{batra2020objectnav}. The approach maintains a semantic map of the explored region and used a learned model to learn semantic priors and predict goal locations to find the target object. Similarly, Gupta et al. \cite{Gupta2019CMP} construct a belief map to use for planning. On the other hand, Yang et al. \cite{Yang2019scenepriors} use a topological representation, constructing an object-to-object knowledge graph and using a graph convolutional network to generate semantic priors. 


\textbf{Semantic Mapping}
One of the fundamental components of SLAM is the construction of a 2D or 3D map. Particularly relevant in the case of object navigation is the incorporation of semantics. Prior works have done so via probabilistic graphical models \cite{bowman2017SemanticSLAM-ProbDataAssoc} or learned computer vision models \cite{zhang2018SemanticSLAM-ObjDetection, Ma2017MultiviewSemanticMap}.
As we follow the work of Chaplot et al. \cite{chaplot2020gose}, we instead use differentiable projection operations, a classic method for transforming 3D point clouds to 2D top-down map.


\textbf{Object Detection}
In addition to planning, object detection is a critical module towards success. Recent works have generally drawn upon pre-trained models from the computer vision community, mostly from semantic segmentation. For example, Chaplot et al. \cite{chaplot2020gose} use Mask-RCNN \cite{he2017mask} and DeepLabv3  \cite{chen2017deeplabv3}, whereas Ye et al. \cite{ye2021auxiliary} use RedNet \cite{jiang2018rednet}. 
Additionally, with the increased interest in embodied tasks in recent years, video semantic segmentation has also become a field of interest. Classic semantic segmentation models do not necessarily perform as well in such an environment, as per-frame predictions can produce inconsistent results across time. Some prior works have tried to improve accuracy by exploiting these temporal relationships, such as \cite{Nilsson2018SemVideoSegGRU} and \cite{zhu17dff}, which use optical flow networks to propagate predictions. More recently, Liu et al. (2020) \cite{Liu2020EfficientSV} instead incorporates temporal consistency as a component of the loss and via knowledge distillation during training. Similarly, Wang et al. (2021)\cite{Wang2021TemporalMA} construct a memory and use attention to relate the current frame and previous frames. While we leave incorporating such techniques to future works, we try to improve temporal consistency via an additional learned model that refines the single-frame object detection system used in \cite{chaplot2020gose}.

==> [IROS 2022] Stubborn_Object_Navigation/backup_results.tex <==


\section{Results}


\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Methods}          & \textbf{Collision Avoidance Update} & \textbf{chair } & \textbf{sofa} & \textbf{bed}  & \textbf{plant} & \textbf{toilet} & \textbf{tv}               & \textbf{average \%}         \\ \hline
\textbf{Frontier}         & \checkmark                          & 75            & 65          & 24          & 56           & 29            & \textbf{100} & $58 \pm 6$          \\ \hline
\multirow{2}{*}{\textbf{SemExp}}   & \xmark                              & 76            & 65          & 38          & 51           & 26            & 83                      & $57\pm 7$           \\
                          & \checkmark                          & 79            & 65          & 38          & 57           & 26            & 83                      & $58\pm 6$           \\ \hline
\multirow{2}{*}{\textbf{Stubborn}} & \xmark                              & 74            & 58          & 38          & 50            & 36            & 66                      & $54 \pm 6$          \\
                          & \checkmark                          & \textbf{80}    & \textbf{72} & \textbf{39} & \textbf{61}  & \textbf{67}   & 83                      & \textbf{67} $\pm 6$ \\ \hline
\end{tabular}
}
\caption{\small GT Exploration Rate in percentage that measures the exploration performance of Frontier, SemExp, and Stubborn. SemExp and Stubborn are both tested with and without the Collision Avoidance Update described in Sec. \ref{ssec:collision-avoidance}}
\label{tab:performance3}
\end{table}



We evaluate the performance gain of each design in terms of exploration efficiency, collision avoidance, and object identification. Also, we present the Stubborn Agent's performance on the Habitat Challenge \cite{savva2019habitat} in Sec.~\ref{Habitat}. In the follow sections, we evaluate the agents' performance in the following two metrics:

\begin{itemize} [wide, labelwidth=!, labelindent=0pt]
    \item \textbf{Ground Truth (GT) Exploration Rate} This metric is used to measure the performance of an exploration strategy. It isolates exploration from other factors that affect success (e.g., object detection and object localization). An agent is considered successful upon the target object occupies at least $0.8\%$ of the pixels in the ground truth semantic mask of the agent's view.
    \item \textbf{Trapped Rate} The agent is considered trapped if it fails to move more than $1$ meter in $100$ time steps. Lower trapped rate is better.
\end{itemize}

\subsection{Exploration Efficiency}
\label{EEResult}

We evaluate the exploration strategy of the Stubborn Agent using GT Exploration Rate. Table \ref{tab:performance3} compares the Stubborn Agent with the baselines. We use SemExp\cite{chaplot2020gose} and the Frontier Based Exploration \cite{frontier}, a classic baseline exploration strategy where robots always try to navigate to the intersections of observed and unobserved space (the frontier), as baselines. We run SemExp with the pre-trained model that is publicly released, but change the global map size of SemExp to $7200\times 7200$ to match with Stubborn. \footenote{Since SemExp released version was intended to be tested on the Gibson dataset\cite{xia2018gibson}, whose indoor scenes are much smaller than Matterport 3D, the original global map size in the released version of SemExp is $2400\times 2400$, which is too small for Matterport 3D dataset. As a result, original SemExp agent is unable to plan path outside of the map of size $2400\times 2400$, resulting in poor exploration}. While Stubborn requires training data for its Object Detection Module, the Object Detection Module is not relevant when using GT Exploration Rate as metrics, so both Frontier and Stubborn Agent requires no training. 

For both SemExp and Stubborn, we evaluate the performance of those agents both with and without the Collision Avoidance Update described in Sec. \ref{ssec:collision-avoidance}. Since one of the baseline methods, SemExp, only supports $6$ semantic categories in its publicly released version, we perform experiments only on those $6$ categories: ``chair'', ``couch'', ``plant'', ``bed'', ``toilet'', ``tv''. The Stubborn Agent with the collision avoidance update outperforms all baselines by a considerable margin and the difference in success rate is statistically significant. The experiments are performed with no constraint on execution time the agents can take. In the Habitat Challenge, where total execution time is constrained (42 hours for 2000 tasks), the Stubborn Policy would perform even better, as it takes $43\%$ less time per step compared to SemExp, allowing it to take more steps with the same time constraint.


\noindent
\textbf{Comparing Stubborn and SemExp} The Stubborn Agent performs similarly with SemExp when both agents are without the collision avoidance update, but performs much stronger when both agents receive the collision avoidance update. This is because the Stubborn Agent gets trapped more easily since its goal is fixed, which forces the agent to go to the corners of the rooms more often. Therefore the Stubborn Agent benefited more from the Collision Avoidance Update, as demonstrated in Fig. \ref{fig:plateau_rate}.




\subsection{Collision Avoidance}
\label{ssec:collision-avoidance}

\begin{table}[t!]
\centering
\caption{\small The four methods used to avoid collisions help the \stubborn Agent reduces the trap rate and improves exploration efficiency measured by the GT exploration rate. The full defnition of abbreviated method names can be found in Sec.~\ref{ssec:collision-avoidance}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|cccc|cc|}
\hline
               & \multicolumn{4}{c|}{\textbf{Collision Avoidance Update}}                   & \multicolumn{2}{c|}{\textbf{Performance}}            \\ \hline
\textbf{Agent} & \textbf{BFUntrap} & \textbf{ColObs} & \textbf{ColAver} & \textbf{VisPath} & \textbf{Trapped\%} & \textbf{GT Exploration Rate \%} \\ \hline
\textbf{I}     &                   &                  &                  &                  & 10.0                 & 54                         \\ \hline
\textbf{II}    & \checkmark        &                  &                  &                  & 8.7                 & 59                         \\ \hline
\textbf{III}   & \checkmark        & \checkmark       &                  &                  & 6.7                 & 64                         \\ \hline
\textbf{IV}    & \checkmark        & \checkmark       & \checkmark       &                  & 5.2                 & 64                         \\ \hline
\textbf{V}     & \checkmark        & \checkmark       & \checkmark       & \checkmark       & \textbf{5.0}        & \textbf{67}                \\ \hline
\end{tabular}
}
\label{tab:stubborn-ablation}
\end{table}


The Stubborn Agent used $4$ methods to decrease failures caused by the agent getting trapped: (i) Brute Force Untrap (BFUntrap; Sec.~\ref{sec:path-planner}); (ii) use of multi-Scale collision obstacle maps ({ColObs}; Sec.~\ref{sec:path-planner}); (iii) collision aversion in exploration planner (ColAver; Sec.~\ref{sec:exploration-module}); and (iv) marking visited paths to as free space (VisPath; Sec.~\ref{sec:mapping}). The importance of each of these contributions is reported in Table~\ref{tab:stubborn-ablation}. The results clearly indicate that all four factors are essential for reducing the trap rate and improving exploration. The most significant performance gain results from multi-scale collisions representation (ColObs). 

%We present an ablation analysis to show how much improvement each method made. Table \ref{tab:stubborn-ablation} shows the performance of the Stubborn Agent with different ablations on the collision avoidance update. All of the $4$ collision avoidance strategies decreased the trapped rate and improved the GT exploration rate, with the biggest improvement made by maintaining two versions of the collision obstacle map (ObsSize).


\begin{figure}
\centering
    \includegraphics[width=.45\textwidth]{images/PlateauRate.png}\hfill
    \caption{\small Trapped Rate of the SemExp Agent and the Stubborn Agent before and after the Collision Avoidance Update. The lower the Trapped Rate is, the better. Stubborn benefited from Collision Avoidance Update more than SemExp did.}
    \label{fig:plateau_rate}
\end{figure}


\subsection{Object Identification}
\label{OIR}
\noindent
\textbf{Training} We use the Naive Bayes Classifier as the binary classifier described in Sec. \ref{sec:object-detection-module}. We collect training data using the validation episodes of Matterport 3D. We collect training data in the validation episode instead of the training episode because the training episodes are already used to train the object segmentation model and therefore not accurate indicators of how the object segmentation model behaves in the testing split. 

We train a separate Naive Bayes Classifier for each target object category and each testing scene. The Classifier for an target object category only uses data gathered from the target object category for training, while the classifier for a testing scene excludes data gathered from the scene to prevent training and testing on the same scene.



\noindent
\textbf{Baseline} We compare the Stubborn agent with a single frame baseline (Single-Frame). Single-Frame differs from the Stubborn agent only in the object detection module: it uses the simple object detection baseline that is similar to SemExp described at the beginning of Sec. \ref{sec:object-detection-module}, where the agent uses the maximum confidence score reported by the semantic segmentation model in each single frame as the only indicator for whether the goal is found.

\noindent
\textbf{Results} We consider results only from target object categories that appeared in more than $4$ scenes in the $2000$ validation episodes to make sure the classifier is trained with sufficient data. Among the $21$ object categories, $15$ of them satisfied the requirement. Results are presented in Table \ref{tab:ObjIDResults}. The agent has increased performance in most categories with the detection module update, but not all categories. Overall, the agent performance increased by about $7\%$. On the Habitat Challenge, the agent's success rate also increased from $22.2\%$ to $23.7\%$, showing that the improvement is consistent in different settings.


\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Goal}               & \textbf{Stubborn \%} & \textbf{Single-Frame \%}  & \textbf{Improvement \%} \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{stool}              & \textbf{16}     & 9            & 77.78                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{toilet}             & \textbf{43}     & 35            & 22.86                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{sink}               & \textbf{31}     & 26            & 19.23                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{chest\_of\_drawers} & \textbf{19}     & 16            & 18.75                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{plant}              & \textbf{33}     & 28            & 17.86                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{bed}                & \textbf{51}     & 44            & 15.91                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{cabinet}            & \textbf{34}     & 30             & 13.33                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{table}              & \textbf{61}     & 56            & 8.93                    \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{counter}            & \textbf{39}     & 36            & 8.33                    \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{chair}              & \textbf{47}     & 46            & 2.17                    \\ \hline
\rowcolor[HTML]{F6F7D9} 
\textbf{sofa}               & 31              & 31            & 0                       \\ \hline
\rowcolor[HTML]{F6F7D9} 
\textbf{seating}            & 69              & 69            & 0                       \\ \hline
\rowcolor[HTML]{F8DFDF} 
\textbf{picture}            & 27              & \textbf{30}    & -10                     \\ \hline
\rowcolor[HTML]{F8DFDF} 
\textbf{cushion}            & 46              & \textbf{56}   & -17.86                  \\ \hline
\rowcolor[HTML]{F8DFDF} 
\textbf{towel}              & 12              & \textbf{15}   & -20                     \\ \hline
\textbf{Average}            & \textbf{37} $\pm 3$   & $35 \pm 3$ & 6.55                   \\ \hline
\end{tabular}
}
\caption{\small Success Rate of Stubborn and Single-Frame Agent on $15$ semantic categories. Categories with improvements are marked green, while categories with worse performance are marked red.}
\label{tab:ObjIDResults}
\end{table}


\subsection{Performance on the Habitat Challenge}
\label{Habitat}
We evaluate the Stubborn Agent on the 2021 Habitat Object Navigation Challenge with the test-standard split. Results in Table \ref{tab:Habitat} show that our agent has the best performance in SPL and the second best performance in Success Rate.

\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l c c|}
\hline
Models                            & \textbf{SPL}    & \textbf{Success Rate \%} \\ \hline
\rowcolor{LightCyan}
(1) yuumi\_the\_magic\_cat(Our Method) & \textbf{0.098}  & 23.7        \\ 
(2) PONI (PF)                        & 0.088  & 20          \\ 
(3) TreasureHunt\cite{maksymets2021thda}                     & 0.087  & 21.1        \\ 
(4) Habitat on Web (IL-HD)           & 0.082  & \textbf{24.4}        \\
(5) EmbCLIP \cite{Khandelwal2021objectnav-clip}                       & 0.078  & 18.1        \\ 
\rowcolor{LightYellow}
(6) Arnold (SemExp)$^{2020}$ \cite{chaplot2020gose}                 & 0.0707 & 17.85       \\ 
(7) Red Rabbit 6-Act Base (EEAux)$^{2021}$ \cite{ye2021auxiliary}          & 0.062  & 23.7        \\  \hline
\end{tabular}
}
\caption{\small \textbf{2021 Habitat Object Navigation Challenge} We report the leaderboard entries on the Test Standard split. Entries with the superscript 2020 and 2021 indicate challenge winners in the corresponding year. Our Method (named Yuumi\_the\_magic\_cat) is first in SPL and second in Success Rate, with a large improvement from SemExp which we built upon.}
\label{tab:Habitat}
\end{table}

==> backup_related_work.tex <==

\section{Related Work}
\label{sec:related-work}

%Two lines of work have been developed to exploit semantics for efficient exploration: (i) constructing an occupancy map using SLAM~\cite{cadena2016past} where every location is labelled with one out of N predefined semantic categories. Such a map is leveraged to set exploration goals for the agent~\cite{chaplot2020gose,Yang2019scenepriors}. (ii) The second approach is end-to-end and predicts actions directly from the raw RGBD observation, the image segmented into several object categories and other metadata~\cite{ye2021auxiliary,Khandelwal2021objectnav-clip, maksymets2021thda,Mousavian2019VisualRF,Wahid2020objectnav-sac}. 

%To find the goal object in an unseen environment, the agent needs to explore the environment, infer goal object locations, and identify the goal object. We briefly discuss prior work on the task of object navigation, as well as related work on semantic maps and object detection.

\textbf{Object Navigation}
Some recent works have approached object navigation via end-to-end imitation or reinforcement learning approaches while implicitly learning semantic priors within the models. Ye et al.~\cite{ye2021auxiliary} learn a policy via reinforcement learning with auxiliary learning tasks and an exploration reward. Khandelwal et al. \cite{Khandelwal2021objectnav-clip} incorporate Contrastive language image pretraining(CLIP, a type of neural network encoder) features for object navigation. Furthermore, Maksymets et al. \cite{maksymets2021thda} augment scenes by inserting objects to increase object and trajectory diversity during training. Mousavian et al. \cite{Mousavian2019VisualRF} use imitation learning to learn a policy. Wahid et al. \cite{Wahid2020objectnav-sac} address the similar problem of object navigation with continuous control using Soft Actor-Critic \cite{Haarnoja2018SAC}.

In contrast, other works have built explicit spatial representations that are then used in navigation, such as a map of the explored region in Simultaneous Localization And Mapping\cite{durrant2006simultaneous}. Chaplot et al. \cite{chaplot2020gose} propose a hierarchical SLAM-based approach, winning the 2020 iteration of the Habitat Challenge \cite{batra2020objectnav}. The approach maintains a semantic map of the explored region and used a learned model to learn semantic priors and predict goal locations to find the target object. Similarly, Gupta et al. \cite{Gupta2019CMP} construct a belief map to use for planning. On the other hand, Yang et al. \cite{Yang2019scenepriors} use a topological representation, constructing an object-to-object knowledge graph and using a graph convolutional network to generate semantic priors. 


\textbf{Semantic Mapping}
One of the fundamental components of SLAM is the construction of a 2D or 3D map. Particularly relevant in the case of object navigation is the incorporation of semantics. Prior works have done so via probabilistic graphical models \cite{bowman2017SemanticSLAM-ProbDataAssoc} or learned computer vision models \cite{zhang2018SemanticSLAM-ObjDetection, Ma2017MultiviewSemanticMap}.
As we follow the work of Chaplot et al. \cite{chaplot2020gose}, we instead use differentiable projection operations, a classic method for transforming 3D point clouds to 2D top-down map.


\textbf{Object Detection}
In addition to planning, object detection is a critical module towards success. Recent works have generally drawn upon pre-trained models from the computer vision community, mostly from semantic segmentation. For example, Chaplot et al. \cite{chaplot2020gose} use Mask-RCNN \cite{he2017mask} and DeepLabv3  \cite{chen2017deeplabv3}, whereas Ye et al. \cite{ye2021auxiliary} use RedNet \cite{jiang2018rednet}. 
Additionally, with the increased interest in embodied tasks in recent years, video semantic segmentation has also become a field of interest. Classic semantic segmentation models do not necessarily perform as well in such an environment, as per-frame predictions can produce inconsistent results across time. Some prior works have tried to improve accuracy by exploiting these temporal relationships, such as \cite{Nilsson2018SemVideoSegGRU} and \cite{zhu17dff}, which use optical flow networks to propagate predictions. More recently, Liu et al. (2020) \cite{Liu2020EfficientSV} instead incorporates temporal consistency as a component of the loss and via knowledge distillation during training. Similarly, Wang et al. (2021)\cite{Wang2021TemporalMA} construct a memory and use attention to relate the current frame and previous frames. While we leave incorporating such techniques to future works, we try to improve temporal consistency via an additional learned model that refines the single-frame object detection system used in \cite{chaplot2020gose}.

==> backup_results.tex <==


\section{Results}


\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Methods}          & \textbf{Collision Avoidance Update} & \textbf{chair } & \textbf{sofa} & \textbf{bed}  & \textbf{plant} & \textbf{toilet} & \textbf{tv}               & \textbf{average \%}         \\ \hline
\textbf{Frontier}         & \checkmark                          & 75            & 65          & 24          & 56           & 29            & \textbf{100} & $58 \pm 6$          \\ \hline
\multirow{2}{*}{\textbf{SemExp}}   & \xmark                              & 76            & 65          & 38          & 51           & 26            & 83                      & $57\pm 7$           \\
                          & \checkmark                          & 79            & 65          & 38          & 57           & 26            & 83                      & $58\pm 6$           \\ \hline
\multirow{2}{*}{\textbf{Stubborn}} & \xmark                              & 74            & 58          & 38          & 50            & 36            & 66                      & $54 \pm 6$          \\
                          & \checkmark                          & \textbf{80}    & \textbf{72} & \textbf{39} & \textbf{61}  & \textbf{67}   & 83                      & \textbf{67} $\pm 6$ \\ \hline
\end{tabular}
}
\caption{\small GT Exploration Rate in percentage that measures the exploration performance of Frontier, SemExp, and Stubborn. SemExp and Stubborn are both tested with and without the Collision Avoidance Update described in Sec. \ref{ssec:collision-avoidance}}
\label{tab:performance3}
\end{table}



We evaluate the performance gain of each design in terms of exploration efficiency, collision avoidance, and object identification. Also, we present the Stubborn Agent's performance on the Habitat Challenge \cite{savva2019habitat} in Sec.~\ref{Habitat}. In the follow sections, we evaluate the agents' performance in the following two metrics:

\begin{itemize} [wide, labelwidth=!, labelindent=0pt]
    \item \textbf{Ground Truth (GT) Exploration Rate} This metric is used to measure the performance of an exploration strategy. It isolates exploration from other factors that affect success (e.g., object detection and object localization). An agent is considered successful upon the target object occupies at least $0.8\%$ of the pixels in the ground truth semantic mask of the agent's view.
    \item \textbf{Trapped Rate} The agent is considered trapped if it fails to move more than $1$ meter in $100$ time steps. Lower trapped rate is better.
\end{itemize}

\subsection{Exploration Efficiency}
\label{EEResult}

We evaluate the exploration strategy of the Stubborn Agent using GT Exploration Rate. Table \ref{tab:performance3} compares the Stubborn Agent with the baselines. We use SemExp\cite{chaplot2020gose} and the Frontier Based Exploration \cite{frontier}, a classic baseline exploration strategy where robots always try to navigate to the intersections of observed and unobserved space (the frontier), as baselines. We run SemExp with the pre-trained model that is publicly released, but change the global map size of SemExp to $7200\times 7200$ to match with Stubborn. \footenote{Since SemExp released version was intended to be tested on the Gibson dataset\cite{xia2018gibson}, whose indoor scenes are much smaller than Matterport 3D, the original global map size in the released version of SemExp is $2400\times 2400$, which is too small for Matterport 3D dataset. As a result, original SemExp agent is unable to plan path outside of the map of size $2400\times 2400$, resulting in poor exploration}. While Stubborn requires training data for its Object Detection Module, the Object Detection Module is not relevant when using GT Exploration Rate as metrics, so both Frontier and Stubborn Agent requires no training. 

For both SemExp and Stubborn, we evaluate the performance of those agents both with and without the Collision Avoidance Update described in Sec. \ref{ssec:collision-avoidance}. Since one of the baseline methods, SemExp, only supports $6$ semantic categories in its publicly released version, we perform experiments only on those $6$ categories: ``chair'', ``couch'', ``plant'', ``bed'', ``toilet'', ``tv''. The Stubborn Agent with the collision avoidance update outperforms all baselines by a considerable margin and the difference in success rate is statistically significant. The experiments are performed with no constraint on execution time the agents can take. In the Habitat Challenge, where total execution time is constrained (42 hours for 2000 tasks), the Stubborn Policy would perform even better, as it takes $43\%$ less time per step compared to SemExp, allowing it to take more steps with the same time constraint.


\noindent
\textbf{Comparing Stubborn and SemExp} The Stubborn Agent performs similarly with SemExp when both agents are without the collision avoidance update, but performs much stronger when both agents receive the collision avoidance update. This is because the Stubborn Agent gets trapped more easily since its goal is fixed, which forces the agent to go to the corners of the rooms more often. Therefore the Stubborn Agent benefited more from the Collision Avoidance Update, as demonstrated in Fig. \ref{fig:plateau_rate}.




\subsection{Collision Avoidance}
\label{ssec:collision-avoidance}

\begin{table}[t!]
\centering
\caption{\small The four methods used to avoid collisions help the \stubborn Agent reduces the trap rate and improves exploration efficiency measured by the GT exploration rate. The full defnition of abbreviated method names can be found in Sec.~\ref{ssec:collision-avoidance}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|cccc|cc|}
\hline
               & \multicolumn{4}{c|}{\textbf{Collision Avoidance Update}}                   & \multicolumn{2}{c|}{\textbf{Performance}}            \\ \hline
\textbf{Agent} & \textbf{BFUntrap} & \textbf{ColObs} & \textbf{ColAver} & \textbf{VisPath} & \textbf{Trapped\%} & \textbf{GT Exploration Rate \%} \\ \hline
\textbf{I}     &                   &                  &                  &                  & 10.0                 & 54                         \\ \hline
\textbf{II}    & \checkmark        &                  &                  &                  & 8.7                 & 59                         \\ \hline
\textbf{III}   & \checkmark        & \checkmark       &                  &                  & 6.7                 & 64                         \\ \hline
\textbf{IV}    & \checkmark        & \checkmark       & \checkmark       &                  & 5.2                 & 64                         \\ \hline
\textbf{V}     & \checkmark        & \checkmark       & \checkmark       & \checkmark       & \textbf{5.0}        & \textbf{67}                \\ \hline
\end{tabular}
}
\label{tab:stubborn-ablation}
\end{table}


The Stubborn Agent used $4$ methods to decrease failures caused by the agent getting trapped: (i) Brute Force Untrap (BFUntrap; Sec.~\ref{sec:path-planner}); (ii) use of multi-Scale collision obstacle maps ({ColObs}; Sec.~\ref{sec:path-planner}); (iii) collision aversion in exploration planner (ColAver; Sec.~\ref{sec:exploration-module}); and (iv) marking visited paths to as free space (VisPath; Sec.~\ref{sec:mapping}). The importance of each of these contributions is reported in Table~\ref{tab:stubborn-ablation}. The results clearly indicate that all four factors are essential for reducing the trap rate and improving exploration. The most significant performance gain results from multi-scale collisions representation (ColObs). 

%We present an ablation analysis to show how much improvement each method made. Table \ref{tab:stubborn-ablation} shows the performance of the Stubborn Agent with different ablations on the collision avoidance update. All of the $4$ collision avoidance strategies decreased the trapped rate and improved the GT exploration rate, with the biggest improvement made by maintaining two versions of the collision obstacle map (ObsSize).


\begin{figure}
\centering
    \includegraphics[width=.45\textwidth]{images/PlateauRate.png}\hfill
    \caption{\small Trapped Rate of the SemExp Agent and the Stubborn Agent before and after the Collision Avoidance Update. The lower the Trapped Rate is, the better. Stubborn benefited from Collision Avoidance Update more than SemExp did.}
    \label{fig:plateau_rate}
\end{figure}


\subsection{Object Identification}
\label{OIR}
\noindent
\textbf{Training} We use the Naive Bayes Classifier as the binary classifier described in Sec. \ref{sec:object-detection-module}. We collect training data using the validation episodes of Matterport 3D. We collect training data in the validation episode instead of the training episode because the training episodes are already used to train the object segmentation model and therefore not accurate indicators of how the object segmentation model behaves in the testing split. 

We train a separate Naive Bayes Classifier for each target object category and each testing scene. The Classifier for an target object category only uses data gathered from the target object category for training, while the classifier for a testing scene excludes data gathered from the scene to prevent training and testing on the same scene.



\noindent
\textbf{Baseline} We compare the Stubborn agent with a single frame baseline (Single-Frame). Single-Frame differs from the Stubborn agent only in the object detection module: it uses the simple object detection baseline that is similar to SemExp described at the beginning of Sec. \ref{sec:object-detection-module}, where the agent uses the maximum confidence score reported by the semantic segmentation model in each single frame as the only indicator for whether the goal is found.

\noindent
\textbf{Results} We consider results only from target object categories that appeared in more than $4$ scenes in the $2000$ validation episodes to make sure the classifier is trained with sufficient data. Among the $21$ object categories, $15$ of them satisfied the requirement. Results are presented in Table \ref{tab:ObjIDResults}. The agent has increased performance in most categories with the detection module update, but not all categories. Overall, the agent performance increased by about $7\%$. On the Habitat Challenge, the agent's success rate also increased from $22.2\%$ to $23.7\%$, showing that the improvement is consistent in different settings.


\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Goal}               & \textbf{Stubborn \%} & \textbf{Single-Frame \%}  & \textbf{Improvement \%} \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{stool}              & \textbf{16}     & 9            & 77.78                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{toilet}             & \textbf{43}     & 35            & 22.86                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{sink}               & \textbf{31}     & 26            & 19.23                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{chest\_of\_drawers} & \textbf{19}     & 16            & 18.75                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{plant}              & \textbf{33}     & 28            & 17.86                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{bed}                & \textbf{51}     & 44            & 15.91                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{cabinet}            & \textbf{34}     & 30             & 13.33                   \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{table}              & \textbf{61}     & 56            & 8.93                    \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{counter}            & \textbf{39}     & 36            & 8.33                    \\ \hline
\rowcolor[HTML]{E4F8E1} 
\textbf{chair}              & \textbf{47}     & 46            & 2.17                    \\ \hline
\rowcolor[HTML]{F6F7D9} 
\textbf{sofa}               & 31              & 31            & 0                       \\ \hline
\rowcolor[HTML]{F6F7D9} 
\textbf{seating}            & 69              & 69            & 0                       \\ \hline
\rowcolor[HTML]{F8DFDF} 
\textbf{picture}            & 27              & \textbf{30}    & -10                     \\ \hline
\rowcolor[HTML]{F8DFDF} 
\textbf{cushion}            & 46              & \textbf{56}   & -17.86                  \\ \hline
\rowcolor[HTML]{F8DFDF} 
\textbf{towel}              & 12              & \textbf{15}   & -20                     \\ \hline
\textbf{Average}            & \textbf{37} $\pm 3$   & $35 \pm 3$ & 6.55                   \\ \hline
\end{tabular}
}
\caption{\small Success Rate of Stubborn and Single-Frame Agent on $15$ semantic categories. Categories with improvements are marked green, while categories with worse performance are marked red.}
\label{tab:ObjIDResults}
\end{table}


\subsection{Performance on the Habitat Challenge}
\label{Habitat}
We evaluate the Stubborn Agent on the 2021 Habitat Object Navigation Challenge with the test-standard split. Results in Table \ref{tab:Habitat} show that our agent has the best performance in SPL and the second best performance in Success Rate.

\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l c c|}
\hline
Models                            & \textbf{SPL}    & \textbf{Success Rate \%} \\ \hline
\rowcolor{LightCyan}
(1) yuumi\_the\_magic\_cat(Our Method) & \textbf{0.098}  & 23.7        \\ 
(2) PONI (PF)                        & 0.088  & 20          \\ 
(3) TreasureHunt\cite{maksymets2021thda}                     & 0.087  & 21.1        \\ 
(4) Habitat on Web (IL-HD)           & 0.082  & \textbf{24.4}        \\
(5) EmbCLIP \cite{Khandelwal2021objectnav-clip}                       & 0.078  & 18.1        \\ 
\rowcolor{LightYellow}
(6) Arnold (SemExp)$^{2020}$ \cite{chaplot2020gose}                 & 0.0707 & 17.85       \\ 
(7) Red Rabbit 6-Act Base (EEAux)$^{2021}$ \cite{ye2021auxiliary}          & 0.062  & 23.7        \\  \hline
\end{tabular}
}
\caption{\small \textbf{2021 Habitat Object Navigation Challenge} We report the leaderboard entries on the Test Standard split. Entries with the superscript 2020 and 2021 indicate challenge winners in the corresponding year. Our Method (named Yuumi\_the\_magic\_cat) is first in SPL and second in Success Rate, with a large improvement from SemExp which we built upon.}
\label{tab:Habitat}
\end{table}
